Sinkhorn Algorithm as a Special Case of Stochastic Mirror Descent

We present a new perspective on the celebrated Sinkhorn algorithm by showing that is a special case of incremental/stochastic mirror descent. In order to see this, one should simply plug Kullback-Leibler divergence in both mirror map and the objective function. Since the problem has unbounded domain, the objective function is neither smooth nor it has bounded gradients. However, one can still approach the problem using the notion of relative smoothness, obtaining that the stochastic objective is 1-relative smooth. The discovered equivalence allows us to propose 1) new methods for optimal transport, 2) an extension of Sinkhorn algorithm beyond two constraints.

==> algs/acc_mirror_descent.tex <==
\begin{algorithm}[t]
\caption{The Extragradient Method for Variational Inequality.}
\label{alg:eg_vi}
\begin{algorithmic}[1]
	\State {\bf Parameters:} $x^0 \in \K$, stepsize $\eta > 0$ 
	\For{$t = 0,1,2,\ldots$}
	\State Sample $\xi^t$
	\State $y^t = \prox{\eta g}{x^t - \eta F(x^t; \xi^t)}$
	\State $x^{t+1} = \prox{\eta g}{x^t - \eta F(y^t; \xi^t)}$
	\EndFor
\end{algorithmic}	
\end{algorithm}
